The Disparate Equilibria of Algorithmic Decision Making when Individuals Invest Rationally

The long-term impact of algorithmic decision making is shaped by the dynamics between the deployed decision rule and individuals' response. Focusing on settings where each individual desires a positive classification---including many important applications such as hiring and school admissions, we study a dynamic learning setting where individuals invest in a positive outcome based on their group's expected gain and the decision rule is updated to maximize institutional benefit. By characterizing the equilibria of these dynamics, we show that natural challenges to desirable long-term outcomes arise due to heterogeneity across groups and the lack of realizability. We consider two interventions, decoupling the decision rule by group and subsidizing the cost of investment. We show that decoupling achieves optimal outcomes in the realizable case but has discrepant effects that may depend on the initial conditions otherwise. In contrast, subsidizing the cost of investment is shown to create better equilibria for the disadvantaged group even in the absence of realizability.

==> 02_eqmmodel.tex <==
% !TeX root = main.tex 


\section{Model of automated decision making with feedback}\label{sec:model}
%
%\subsection{Model}
%
%\paragraph{Setting} Given a candidate with features $X_i \in \calX$, we want to predict their outcome $Y_i \in \{0,1\}$. Original candidate pool distribution $(X, Y) \sim \calP$. Possibly the outcome $y_i$ is only revealed for accepted candidates, but we also make random acceptances to ensure we able to construct unbiased estimators under $\calP_t$.
%
%Suppose we start with a model $\hat{\theta}_0$ and update it with new data collected at every round.
%
%New candidates apply at every round. We now suppose candidates can observe the previous model, and use it to decide whether to apply. In other words, the candidate pool distribution is changing with the model.
%

%\todo{Make not specific to hiring.}


\begin{figure}[htbp]
	\centering
	\begin{tikzpicture}[->,shorten >=1pt,auto,node distance=2cm,
	thick,main node/.style={circle,draw,font=\Large},sub node/.style={font=\Large}]
	
	\node[main node] (Y) {$Y$};
	\node[main node] (X) [below of=Y] {$X$};
	\node[sub node] (D) [left of=Y] {$y(c, \theta)$};
	\node[main node] (A) [above right of=X] {$A$};

	\path[every node/.style={font=\small}]
	(Y) edge node [right] {} (X)
	(D) edge node [right] {} (Y)
	(A) edge node [right] {} (X);
	\end{tikzpicture}
		\begin{tikzpicture}[->,shorten >=1pt,auto,node distance=2cm,
	thick,main node/.style={circle,draw,font=\Large},sub node/.style={font=\Large}]
	
	\node[main node] (Y) {$Y$};
	\node[main node] (X) [below of=Y] {$X$};
	\node[sub node] (D) [left of=X] {$x(c,\theta)$};
	
	\path[every node/.style={font=\small}]
	(Y) edge node [right] {} (X)
	(D) edge node [right] {} (X);
	\end{tikzpicture}
	
	\caption{Causal graph with \emph{do}-interventions for our individual investment model (left) and the strategic manipulation model (right). In the former, the individual intervenes on the node for the outcome (qualification), $Y$, and this indirectly changes the distribution of the features $X$. Note that $X$ is also a child of the group attribute node $A$. In strategic manipulation, the individual intervenes directly on the features, $X$, and this is assumed to have no effect on $Y$. In both cases, the value of the intervention, $y(c,\theta)$ or $x(c,\theta)$, depends on the cost $c$ and the classifier $\theta$.}
	\label{fig:graph-ourmodel}
\end{figure}
\nhcomment{Alternatively, we could define $x\in \calX$ and $a\in \calA$ and then say that $X$ and $A$ are the corresponding random variables. I don't trust the probability savviness of FAT* reviewers in understanding the switch between values and random variables without the expalantion.}


In this section we introduce a model of automated decision making with feedback. 
%the difference between value and random variable and not get confused by but it's possible that somebody that's a bit less savey with probability might find the switch between values and random variables confusing.} 
\nhedit{We consider an instance space $\calX$, where $X\in \calX$ denotes the features of an individual that is observable by the institution. We also consider a label space $\calY = \{0,1\}$ where $Y=1$ indicates that an individual has the qualifications desired by the institution and $Y=0$ otherwise. We denote the set of all protected/group attributes by $\calA$ where $A\in \A$ denotes an individual's protected attribute. 
We denote the group proportions by $n_a := \Pr(A=a)$ for all $a\in \calA$.}

An individual decides whether to acquire qualifications, \nhedit{that is to invest in obtaining label $Y=1$.}\footnote{This can be seen as performing an causal intervention on $Y$, which is typically denoted with the $do$-operator \citep[see e.g.,][]{Pearl:2009:CMR:1642718}. For example, we may write $do(Y=1)$ for making the decision to acquire qualifications. Our model (Figure \ref{fig:graph-ourmodel}, left) assumes that $Y$ is not the child of any node, so we in fact have $\Pr(\cdot \mid do( Y=y)) = \Pr(\cdot \mid Y=y)$. Henceforth we shall drop the $do$-operator whenever we condition on $Y$.}
\nhedit{To get label $Y=1$ an individual from any group has to pay a cost $C$ that is distributed according to CDF $G(\cdot)$. 
A qualified individual from group $a\in \calA$, i.e., one who invested in label $Y=1$, has features $x\in \calX$ with probability $\Pr(X=x \mid Y=1, A=a)$. Similarly, an unqualified individual from group $a\in \calA$ receives features $x$ with probability $\Pr(X=x\mid Y=0, A=a)$.
} 
 
% Let $A \in \calA$ be the protected/group attribute(s), $X \in \calX$ be the features of the individual that the institution can observe, $Y \in \{0,1\}$ be the label of whether the individual has the qualifications desired by the institution.
%
%} where
%$C$ is distributed randomly in each group with CDF, $G(\cdot)$.  

We also consider an institution that is interested in hiring qualified individuals.
Let $\hat{Y}_\theta \in \{0,1\}$ denote the qualification determination, which is parametrized by $\theta \in \Theta$. 


%that The institution gains $p_{\text{TP}} > 0$ for accepting an individual that meets their qualifications and %hiring a skilled candidate and 
%loses $c_{\text{FP}} > 0$ for choosing an individual that does not meet their qualifications. %hiring an unskilled candidate. 
%It accepts an individual to maximize its utility %hiring decision to maximize profit:

%Let the group proportions be $n_a := \Pr(A=a)$.
 
 %\todo{Should use the notation do($Y=1$) at first to show that we condition on the intervention on $Y$. then drop the do() notation once we've established that the only way to affect X is through Y in our model}

\paragraph{Individual's utility maximization} Given the current qualification determination $\hat{Y}_\theta$, an individual from group $a$ acquires the label $Y=1$ if the benefit outweighs the costs: \begin{equation}\label{eq:individ_dec}
w \text{TPR}_a(\theta) - C > w\text{FPR}_a(\theta),
\end{equation}
where $\text{TPR}_a(\theta) = \E[\hat{Y}_\theta\mid  Y=1, A=a]$ and $\text{FPR}_a(\theta)= \E[\hat{Y}_\theta\mid Y=0 , A=a]$ are the true positive and false positive rates of the decision rule in group $a$, respectively,  %and $\text{FPR}_a(\theta)= \E[\hat{Y}_\theta\mid $do$(Y=0) , A=a]$ is the false positive rate of the decision rule in group $a$, so that 
so that $w( \text{TPR}_a(\theta)- \text{FPR}_a(\theta))$ measures the benefit of acquiring the label $Y=1$. Note that $\pi= (\pi_a)_{a\in \calA}$ is a function of $\theta$. Indeed, the fraction of group $a$ that is qualified,
\begin{equation}
\pi_a(\theta) := \Pr(Y=1\mid A=a) = \Pr( C < w (\text{TPR}_a(\theta) - \text{FPR}_a(\theta) ) ) = G(w (\text{TPR}_a(\theta) - \text{FPR}_a(\theta) ))
\end{equation}

A qualified individual from group $a$ has features distributed like $\Pr(X=x \mid Y=1, A=a)$; an unqualified individual has feature distribution, $\Pr(X=x\mid Y=0, A=a)$. Note that the conditional feature distributions differ across group.



\paragraph{Institution's utility maximization} The institution gains $p_{\text{TP}} > 0$ for accepting an individual that meets their qualifications and %hiring a skilled candidate and 
loses $c_{\text{FP}} > 0$ for choosing an individual that does not meet their qualifications. %hiring an unskilled candidate. 
It accepts an individual to maximize its utility %hiring decision to maximize profit:
\begin{equation}\label{eq:instit_dec}
\theta^* \in \argmax_{\theta\in \Theta} ~p_{\text{TP}}\cdot \Pr(\hat{Y}_\theta = 1, Y=1) - c_{\text{FP}}\cdot \Pr(\hat{Y}_\theta = 1, Y=0).
\end{equation}
The identity, 
%Note that 
 \begin{align*}
&\argmax_{\theta\in \Theta} ~p_{\text{TP}}\cdot \Pr(\hat{Y}_\theta = 1, Y=1) - c_{\text{FP}}\cdot \Pr(\hat{Y}_\theta = 1, Y=0) \\
	=&\argmax_{\theta\in \Theta} ~p_{\text{TP}}\cdot \sum_{a\in \calA} \text{TPR}_a(\theta) \cdot \pi_a \cdot n_a -\sum_{a\in \calA} c_{\text{FP}}\cdot \text{FPR}_a(\theta) \cdot (1-\pi_a) \cdot n_a,
\end{align*}
illustrates that the utility maximizing set of parameter $\theta^\ast$ is a function of $\pi $, the current proportion of qualified vs. unqualified people in each group. To ensure the dynamics are well-defined, we assume the existence of the well-defined tie-breaking function so that $\theta^\ast$ is uniquely defined. 



\paragraph{Dynamical system for $\pi$} As described above, given an initial state $\pi(0)$, $\pi$ evolves according to $\pi(t)  = \Phi(\pi({t-1}))$, where $\Phi = \pi \circ \theta^*$. %We assume that  $\theta^\ast$ is a uniquely determined so that $\Phi$ is well-defined. %, , $\Phi$ is not well-defined, and so we. To resolve this issue, we assume \lnote{resolve notation when $\theta^*$ is a set?}%$\dots$  \lnote{resolve notation when $\theta^*$ is a set?}
\paragraph{Equilibria} The system we defined above is at equilibrium if $\pi = \Phi(\pi)$. We call such values of $\pi$ (and their corresponding $\theta$) equilibria, or equivalently, fixed points. When a system reaches a fixed point, it will stay at that value. 

%Interesting questions are:
%\begin{enumerate}
%	\item Are there multiple equilibria? How do we select among them? (e.g. depending on initial conditions)
%	\item Number of equilibria in multi-dimensional $X$ setting, and characterization of $\pi_a$ at these equilibria
%	\item View selection bias as a way of selecting among equilibria and show it can be hard to correct without large changes?
%	\item Does the choice of model class/parametrization have ramifications for the types of equilibria?
%	\item Does a bound on differences in feature distributions give a bound on the group-differences at equilibria?
%	\item Effect of collecting more features on tradeoffs at equilibria?
%	\item Non-realizability within groups (i.e. conditional feature distributions overlap). Realizable within groups but non-realizable overall.
%\end{enumerate}

In general, the fixed points of $\Phi$ are not unique. It is therefore of interest to characterize the possible fixed points of the system and to compare them on several metrics of societal importance.
\begin{enumerate}
	\item {\em Stability:} we might be interested to know where there exists a non-finite number of initial conditions $\pi(0)$ such that $ \pi^\ast = \lim_{n \rightarrow \infty} \Phi^n(\pi(0))$ where $\Phi^n(\pi)$ composes the map $\Phi$ $n$ times and applies the result to $\pi$. We consider such equilibria to be stable. In particular, if there exists a neighborhood around $\pi^*$ such that all points converge to $\pi^*$ under the dynamics, we say that $\pi^*$ is \emph{locally stable}. %:= \underbrace{\Phi \circ \Phi \circ \dots \circ \Phi}_{ n \,\,\text{times}}(\pi)$. %, given these are the equilibria that are feasible to obtain. % unstable equilibria are hard to attain. %The stability of the dynamical system implies that there is a class of models or initial conditions for which the trajectories would be equivalent. 
	\item {\em Investment Level:} we might compare equilibria by the total number of individuals who have decided to invested in qualifications.  
	\item {\em Balance:} given two groups $a_1$ and $a_2$, we might prioritize more balanced equilibria, where we call an equilibria {\em balanced} if $| \pi_{a_1}^\ast - \pi_{a_2}^\ast|=  0$. %and {\em unbalanced} if $| \frac{\pi_{a_1}^\ast}{\pi^\ast} - \frac{\pi_{a_2}^\ast}{\pi^\ast}| =  1$. 
	\item {\em Institutional utility:} we might be interested to understand if the institutional utility maximizing equilibria is alligned with equilibria that are desirable according to other metrics. \end{enumerate}

We now list some examples of real-word dynamics that fit nicely into our setting. 
\begin{example}[Hiring] Consider the hiring setting, where $X$ is the features that the firm can observe, $Y$ is whether the applicant meets the qualifications of the firm, $C$ is the cost of acquiring the qualifications required by the firm, and $Y_\theta$ is the hiring decision. The firm accepts candidates to according to utility assessment involving $p_{\text{TP}}$, the profit from hiring a qualified candidate, and $c_{\text{FP}}$, the cost of hiring an unqualified candidate. The candidate, on the other hand, is incentivized to acquire the qualifications for the job based on~\eqref{eq:individ_dec} based on the wage, $w$, and how noisy the decisions of the hiring firm are for the group the candidate belongs to. 

\end{example}
\begin{example}[College Admissions] Consider the college admission setting, where $X$ is the features that the college can observe, $Y$ is whether the applicant meets the qualifications of the college, $C$ is the cost of investing in the qualifications, and $Y_\theta$ is the decision rule of the college. The college accepts applicants by trading off between the utility gain, $p_{\text{TP}}$, of admitting qualified candidates and utility cost, $c_{\text{FP}}$, of admitting an unqualified candidates. The candidate is incentivized to acquire the qualifications for the college based~\eqref{eq:individ_dec} the long term benefit, $w$, and how noisy the decisions of the college are for the group the candidate belongs to. 
 

% Consider the setting of lending, where $X \in \X$ is the features that the lending agency can observe, $Y=\{0,1\}$ is whether the applicant qualifies for a loan, $C$ is the cost of acquiring the necessary qualifications to receive the loan, and $Y_\theta$ is the lending decision of the agency. In this model, the agency chooses applicants to maximize it profit (i.e. according to , and the candidate works to become qualified for the loan  to receive the loan according to the cost of $C$ 

\end{example}
We also consider a highly stylized example of loaning in Section~\ref{sec:experiments}.
 %
%
%A limitation  between our model and models that might more f is that the decisions made by the institution in our model do can only change the feature distribution among individuals through the label Y, but not directly. 
%This may not faithfully capture more complex dynamics between individuals and decision systems such as recidivism or credit scoring. %.  less clear how inviduals can invest in their labels ahead of time. more complex dyanamics that our model does not capture 
%
%Subsequently, the $\text{do}(\cdot)$ notation in our model is unnecessary. % by providing incentives to invest. 
%
 Note, we have assumed the institution has unbiased estimates of TPR and FPR. While selection bias can be resolved by a small degree of random sampling in theory, it remains a large problem in practice that requires domain specific knowledge. We have also avoid all statistical issues by assuming the institution has a lot of samples from the candidate distribution. We leave finite sample questions related to equilibria to future work.
%\todo{include disclaimer about sampling (we assume the institution have unbiased estimate of TPR and FPR. in theory, selective labeling/selection bias can be resolved by a small degree of random sampling, but this is still a large problem in practice that requires domain specific knowledge/solutions.) and statistical issues (we assume the institution has a lot of samples from the desired distribution. leave finite sample questions related to equilibria to future work)}
\todo{citation for importance sampling}


\paragraph{Related work} %The model in this work is closely related to \citet{coate93will}, with several key distinctions: 
The proposed model of feedback dynamics is closely related to \citet{coate93will}, with several key distinctions: 1)~We assume the institution has access to multiple features $X$ when learning about the qualifications of each individuals, whereas~\citet{coate93will} assume $X$ a one-dimensional `noisy signal.' Our assumption is consistent with standard machine learning applications.
2)~We consider the case where the conditional feature distributions,  $\Pr(X=x \mid Y=1, A=a)$,  differ across groups whereas~\citet{coate93will} does not. Note that if the conditional feature distributions are the same across groups,  then group-blind hiring policies %(using the same model for all groups) 
%are such that all 
results in equilibria where all groups have the same rate of skill acquisition and are hired at the same rate and this does not corroborate with reality. Indeed, most instituions do not explicitly use different models for different groups and yet discriminatory outcomes are observed due to the fact that conditional feature distributions do in fact differ across groups. For example, consider %The reason is that , and we would like to understand the ramifications of these differences.
%\todo{could be a subsection.}
%1)~We consider $X$ as belonging to a multi-dimensional feature space instead of being a one-dimensional `noisy signal'. In typical machine learning applications, we have access to multiple features and the goal is to learn the best signal of skill level from these features. 
%2)~We focus on the case where conditional feature distributions,  $\Pr(X=x \mid Y=1, A=a)$,  differ across groups. Note that if conditional feature distributions are the same across groups, all equilibria for group-blind hiring policies (using the same model for all groups) are such that all groups have the same rate of skill acquisition and are hired at the same rate---this does not corroborate with reality. Firms don't deliberately use different models for different genders (e.g. Amazon's hiring tool) and yet discriminatory outcomes are observed. The reason is that conditional feature distributions do in fact differ across groups, and we would like to understand the ramifications of these differences.
%\todo{could be a subsection.}


%
%\begin{example}[Socially good coupled equilibrium]	Consider two groups $a, a_2$. Suppose $X$ is multi-dimensional score vector, and the conditional distributions of the marginals are uniform. 
%%For simplicity, suppose $d = 2$ so that $X = [X_1, X_2]$. In the fully general setting, we have
%\begin{align*}
%\Pr(X<x \mid Y=1, A=a) = \frac{(x - h_{a,\ell})_+}{h_{a,u}-h_{a,\ell}} \quad \quad & \Pr(X<x \mid Y=0, A=a) = \frac{x }{h_{a,\ell}} + \frac{x- h_{a,u}}{1-h_{a,u}}\\
%%\Pr(X_2<x \mid Y=1, A=a) = \frac{(x - h_{a,2,\ell})_+}{h_{a,2,u}-h_{a,2,\ell}} \quad \quad & \Pr(X<x \mid Y=0, A=a) =  \frac{x- h_{a,2,u}}{1-h_{a,2,u}}
%%\end{align*}
%%for group $a$ where $0 < h_{a,i,\ell} < h_{a,i,u} < 1$ for $i = 1,2$; and similarly for group $a_2$
%%\begin{align*}
%\Pr(X<x \mid Y=1, A=a_2) = \frac{(x - h_{a_2,\ell})_+}{h_{a_2,u}-h_{a_2,\ell}} \quad \quad & \Pr(X<x \mid Y=0, A=a_2) = \frac{x }{h_{a_2,\ell}} + \frac{x- h_{a_2,u}}{1-h_{a_2,u}}\\
%%\Pr(X_2<x \mid Y=1, A=a_2) = \frac{(x - h_{a_2,2,\ell})_+}{h_{a_2,2,u}-h_{a_2,2,\ell}} \quad \quad & \Pr(X<x \mid Y=0, A=a_2) = \frac{x }{h_{a_2,2,\ell}} + \frac{x- h_{a_2,2,u}}{1-h_{a_2,2,u}}
%\end{align*}
%where $0<h_{a,\ell} <h_{a_2,\ell}< h_{a, u} < h_{a_2,u}<1$.
%%where $0 < h_{a_2,i,\ell} < h_{a_2,i,u} < 1$ for $i = 1,2$. However, we make the following simplifying assumptions: 
%%\begin{align}
%%h_{a,1,u} &= h_{a_2,1,u} = 1 \qquad\qquad  h_{a,1,\ell} = h_{a_2,1,\ell}:= h_{1,\ell},\\
%% 0= h_{a,2,\ell} &<h_{a_2,2,\ell} \qquad\qquad h_{a,2, u} < h_{a_2,2,u} = 1 
%%\end{align}
%% so that, 
%%\begin{align*}
%%\Pr(X_1<x \mid Y=1, A=a) = \frac{(x - h_{1,\ell})_+}{1-h_{1,\ell}} \quad \quad & \Pr(X<x \mid Y=0, A=a) = \frac{x }{h_{1,\ell}} \\
%%\Pr(X_2<x \mid Y=1, A=a) = \frac{x }{h_{a,2,u}} \quad \quad & \Pr(X<x \mid Y=0, A=a) = \frac{x }{h_{a,2,\ell}} + \frac{x- h_{a,2,u}}{1-h_{a,2,u}}
%%\end{align*}
%%and %for group $a$ where $0 < h_{a,i,\ell} < h_{a,i,u} < 1$ for $i = 1,2$; and similarly for group $a_2$
%%\begin{align*}
%%\Pr(X_1<x \mid Y=1, A=a_2) = \frac{(x - h_{1,\ell})_+}{1-h_{1,\ell}} \quad \quad & \Pr(X<x \mid Y=0, A=a_2) = \frac{x }{h_{1,\ell}}\\
%%\Pr(X_2<x \mid Y=1, A=a_2) = \frac{(x - h_{a_2,2,\ell})_+}{1-h_{a_2,2,\ell}} \quad \quad & \Pr(X<x \mid Y=0, A=a_2) = \frac{x }{h_{a_2,2,\ell}} 
%%\end{align*}
%%%
%%%
%%%
%Consider the set of thresholds $\hat Y_{h_\ell, h_u} =\Ind{h_u>X_1> h_\ell}$ where $h_u,h_\ell\in [0,1]$ is the class of policy parameters. Then for our simple case, there exists three equlibria at %\dots [fill in details]
%%
%\begin{proof} First consider $\hat Y = \Ind{h_{a,\ell}<X<h_{a,u}}$. Then $\pi_a = G(w)$ and $\pi_{a_2} = G(w \left(\frac{h_{a,u} - h_{a,\ell}}{h_{a_2,u} - h_{a,\ell} } - \frac{h_{a_2,\ell} - h_{a,\ell}}{1 + h_{a,\ell} - h_{a_2,u}}\right)  )$. As in our previous example,  $\hat{Y}_1$ is optimal for this $\pi$ if the gain from true positives in group $a$ offsets the loss from false positives in group $a_2$ for $X \in  [h_{a,u}, h_{a_2u}]$, i.e. we need 
%\begin{align}
%\frac{G(w)\cdot n_a \cdot p_{TP}}{h_{a,u} - h_{a,\ell} } >\frac{( 1- G(w \left(\frac{h_{a,u} - h_{a,\ell}}{h_{a_2,u} - h_{a,\ell} } - \frac{h_{a_2,\ell} - h_{a,\ell}}{1 + h_{a,\ell} - h_{a_2,u}}\right)  ) \cdot n_a \cdot c_{FP}}{ }
%\end{align}
%
%Second, consider $\hat Y = \Ind{h_{a_2,\ell}<X<h_{a_2,u}}$. Then $\pi_{a_2} = G(w)$ and $\pi_{a_2} = G(w \left(\frac{h_{a,u} - h_{a,\ell}}{h_{a_2,u} - h_{a,\ell} } - \frac{h_{a_2,\ell} - h_{a,\ell}}{1 + h_{a,\ell} - h_{a_2,u}}\right)  )$
%%
%%
%%Second, consider $\hat Y = \Ind{X_1> h_{1\ell}}\Ind{h_{a_2,2,u}>X_2 >h_{a_2,2,\ell}}$ 
%%
%%Third, consider the case where $h_{a_2,2,u} \neq h_{a,2,u}$
%\end{proof}
%Now lets check that these conditions holde for $G(w) =w$, $n_a \cdot p_{TP} = n_{a_2} \cdot c_{FP}$, 
%%
%
%\end{example} 






==> 02_problem_setting.tex <==
% !TeX root = main.tex 

\section{Background}

Many of the harms, as well as challenges, of applying machine learning in real world contexts have been attributed, at least partly, to various forms of non-stationarity, including ``feedback loops'', where the presently deployed model changes the distribution of future data which is later used to update the model, via retraining. In order to align decisions made by automated data-driven systems with desirable long-term societal outcomes, we need to better understand the impact of these algorithms through time.

%As a result, several authors have come up with models of feedback and dynamics, especially in the fair machine learning setting. These models tend to be specific to effects that the authors want to study and it is not clear how to relate them to each other. It is also not clear what the differences and deficiencies of the models are etc. What other types of feedback are not captured, and that we need to be aware of?

Our goal is to advance a framework for reasoning about feedback loops in machine learning systems that interact with a possibly changing distribution of users.%, so that intuitions can be put on a firm mathematical foundation or falsified within reasonable models. 

We are interested in types of feedback that have not been explored by previous work \citep{Hu2018shortterm,liu18delayed, hashimoto18demographics, Mouzannar2019socialequality, Kilbertus19Fair}, such as
	\begin{enumerate}
		\item Classifier is retrained on data that has selection bias due to previous application of classifier. The way to debias the empirical loss is to apply inverse-propensity score weighting, and to assume the sampling distribution has positive measure w.r.t. the reference distribution, i.e. `exploring policies' \citep{Kilbertus19Fair}.
		\item False negatives have a larger delayed harm by reducing the incentive for individuals to participate in the future
		\item Small initial bias in classifier can be amplified. Would this lead to eventual segregation of two groups? (e.g. there are two classifiers and each ends up serving a different group)
	\end{enumerate}

%\paragraph{Notation} Consider a classifier $c_{\theta}^{(t)}(x)$ at time $t$ parameterized by $\theta$ that takes in features $x$. It is trained with loss $\ell(\theta, x, y)$ on empirical data. There are $k$ groups (commonly $k=2$), and for group $k$, we have $Z=(X, Y) \sim \calP_k$. 



\subsection{Model}

\paragraph{Setting} Given a candidate with features $X_i \in \calX$, we want to predict their outcome $Y_i \in \{0,1\}$. Original candidate pool distribution $(X, Y) \sim \calP$. Possibly the outcome $y_i$ is only revealed for accepted candidates, but we also make random acceptances to ensure we able to construct unbiased estimators under $\calP_t$.

Suppose we start with a model $\hat{\theta}_0$ and update it with new data collected at every round.

New candidates apply at every round. We now suppose candidates can observe the previous model, and use it to decide whether to apply. In other words, the candidate pool distribution is changing with the model.



